Inference for Nonlinear Endogenous Treatment Effects Accounting for High-Dimensional Covariate Complexity

Nonlinearity and endogeneity are prevalent challenges in causal analysis using observational data. This paper proposes an inference procedure for a nonlinear and endogenous marginal effect function, defined as the derivative of the nonparametric treatment function, with a primary focus on an additive model that includes high-dimensional covariates. Using the control function approach for identification, we implement a regularized nonparametric estimation to obtain an initial estimator of the model. Such an initial estimator suffers from two biases: the bias in estimating the control function and the regularization bias for the high-dimensional outcome model. Our key innovation is to devise the double bias correction procedure that corrects these two biases simultaneously. Building on this debiased estimator, we further provide a confidence band of the marginal effect function. Simulations and an empirical study of air pollution and migration demonstrate the validity of our procedures.

==> Lindeberg.tex <==
Define $\zeta_i:=\dfrac{\hat m^\top \hat F_\ic \varepsilon_i} {\sqrt{n_b}\cdot\sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}}$. Then for all $i\in\Nb$, $\zeta_i$ are independent conditional on $\{v,X,Z,\mathcal{F}_a\}$ with 
 \[\E\left(\zeta_i|v,X,Z,\mathcal{F}_a\right)=0,\ \sumb\E\left(\zeta_i^2|v,X,Z,\mathcal{F}_a\right)=1.\]
 It suffices to show the Lindeberg condition holds. Note that 
 \[|\zeta_i| \leq \dfrac{\|\hat F\hat m\|_\infty\cdot |\varepsilon_i|}{\sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}} \leq \dfrac{M^\nu\|B^\prime(d_0)\|_2\cdot |\varepsilon_i|}{\sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}}.\]
 Consequently, for any $\epsilon > 0$
 \[\begin{aligned}
     &\ \ \ \ n_b^{-1}\sumb \E\left(\zeta_i^2\textbf{1}\left\{|\zeta_i|>\epsilon\sqrt{n_b}\right\}\Bigg|v,Z,X,\mathcal{F}_a\right)\\
     &\leq n_b^{-1}\sumb \E\left(\zeta_i^2\textbf{1}\left\{|\varepsilon_i|>\dfrac{\epsilon\sqrt{n_b}\cdot \sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}}{M^\nu\|B^\prime(d_0)\|_2}\right\}\Bigg|v,Z,X,\mathcal{F}_a\right)\\
      &= n_b^{-1}\sumb \dfrac{\hat m^\top\hat F_\ic \hat F_\ic^\top \hat m}{\hat m^\top\hat\Sigma_F \hat m}\E\left(\dfrac{\varepsilon_i^2}{\sigma_\varepsilon^2}\textbf{1}\left\{|\varepsilon_i|>\dfrac{\epsilon\sqrt{n_b}\cdot  \sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}}{M^\nu\|B^\prime(d_0)\|_2}\right\}\Bigg|v,Z,X,\mathcal{F}_a\right)\\
      &=  \E\left(\dfrac{\varepsilon_1^2}{\sigma_\varepsilon^2}\textbf{1}\left\{|\varepsilon_1|>\dfrac{\epsilon\sqrt{n_b}\cdot  \sigma_\varepsilon\sqrt{\hat m^\top\hat\Sigma_F\hat m}}{M^\nu\|B^\prime(d_0)\|_2}\right\}\Bigg|v,Z,X,\mathcal{F}_a\right)\\
      &\leq \left[ \dfrac{M^\nu\|B^\prime(d_0)\|_2}{\epsilon\sqrt{n_b}\cdot\sqrt{\hat m^\top\hat\Sigma_F\hat m}}\right]^\tau\cdot\E\left(\dfrac{\varepsilon_1^{2+\tau}}{\sigma_\varepsilon^{2+\tau}} \Bigg|v,Z,X,\mathcal{F}_a\right) \lep \left(\dfrac{M^\nu}{\epsilon\sqrt{nM}}\right)^\tau \convp 0.\\
 \end{aligned}\]

==> Tables/Simul.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\begin{center} 
\caption{Simulation Results}
\label{tab:simul}
\begin{tabular}{cccccc}
\hline\hline 
$p_x$                   & $n$    & $100\times$BiasInit & $100\times$BiasDB & Coverage & Length \\
\hline 
\multicolumn{6}{c}{$g(d) = 0$}                                        \\
\hline 
\multirow{3}{*}{150} & 500  & 3.100    & 2.758  & 0.980    & 1.757  \\
                     & 750  & 0.942    & 0.883  & 0.972    & 1.039  \\
                     & 1000 & 1.152    & 0.678  & 0.976    & 0.784  \\
\multirow{3}{*}{800} & 500  & 2.880    & 2.586  & 0.894    & 0.665  \\
                     & 750  & 0.842    & 0.890  & 0.934    & 0.749  \\
                     & 1000 & 1.575    & 1.125  & 0.948    & 0.714  \\
                     \hline 
\multicolumn{6}{c}{$g(d) = 0.05(d-3)^3$}                                     \\
\hline 
\multirow{3}{*}{150} & 500  & 3.163    & 2.697  & 0.980    & 1.755  \\
                     & 750  & 1.080    & 0.884  & 0.972    & 1.040  \\
                     & 1000 & 1.246    & 0.680  & 0.976    & 0.784  \\
\multirow{3}{*}{800} & 500  & 2.924    & 2.553  & 0.896    & 0.665  \\
                     & 750  & 0.949    & 0.750  & 0.934    & 0.749  \\
                     & 1000 & 1.530    & 1.104  & 0.948    & 0.714  \\
                     \hline \hline 
\end{tabular}
\end{center}
{\footnotesize Note: ``BiasInit'' and ``BiasDB'' denote the average bias of the initial Lasso estimator $\hat g^\prime(\cdot)$ and the bias-corrected estimator $\tilde g^\prime(\cdot)$ , respectively. ``Coverage'' shows the coverage probability of the 95\% confidence band defined as \eqref{eq: def confidence band} over 500 replications. ``Length'' stands for the point-wise average length of the confidence band.}
\end{table}
